Probabilistic Forecasting of Irregular Time Series via Conditional Flows

Probabilistic forecasting of irregularly sampled multivariate time series with missing values is an important problem in many fields, including health care, astronomy, and climate. State-of-the-art methods for the task estimate only marginal distributions of observations in single channels and at single timepoints, assuming a fixed-shape parametric distribution. In this work, we propose a novel model, ProFITi, for probabilistic forecasting of irregularly sampled time series with missing values using conditional normalizing flows. The model learns joint distributions over the future values of the time series conditioned on past observations and queried channels and times, without assuming any fixed shape of the underlying distribution. As model components, we introduce a novel invertible triangular attention layer and an invertible non-linear activation function on and onto the whole real line. We conduct extensive experiments on four datasets and demonstrate that the proposed model provides $4$ times higher likelihood over the previously best model.

==> couple_layer_yvk.tex <==
\section{Invariant Conditional Normalizing Flow Models}
\label{sec:inv_cond_flow}
\paragraph{Normalizing flows.}
Parametrizing a specific distribution, such as the Normal,
% TODO: reference
is a simple and robust approach to probabilistic forecasting
that can be added on top of any point forecasting model
(for marginal distributions or fixed-size queries at least).
However, such models are less suited for targets having a more
complex distribution. Then typically normalizing flows are
used \citep{Rippel2013.Highdimensional,Papamakarios2021.Normalizing}.
A normalizing flow is an (unconditional) density model for 
variables $y\in\R^K$ consisting of
a simple base distribution,
typically a standard normal $p_Z(z):= \normal(z; 0_K, \id_{K\times K})$, and
an invertible, differentiable, parametrized map
$f(z; \theta)$; then
\begin{align}
	\hat p(y; \theta) :=
	p_Z(f^{-1}(y; \theta)) \left| \text{det}\left(\frac{\partial f^{-1}(y; \theta)}{\partial y}\right) \right|
	\label{eq:nf}
\end{align}
is a proper density, i.e., integrates to 1, and can be fitted to data minimizing
negative log likelihood via gradient descent algorithms.
A normalizing flow can be conditioned on predictor variables $x\in\R^M$
by simply making $f$ dependent on predictors $x$, too: $f(z; x, \theta)$. 
$f$ then has to be invertible w.r.t. $z$ for any $x$ and $\theta$ \citep{Trippe2018.Conditional}.

\paragraph{Invariant conditional normalizing flows.}
A conditional normalizing flow represents an invariant
conditional distribution in the sense of eq.~\ref{eq:invariant},
if
i) its predictors $x$ also can be grouped into $K$ elements $x_1,\ldots,x_K$
and possibly common elements $x\com$:
$x =(x_1,\ldots,x_K,x\com)$, and
ii) its transformation $f$ is equivariant in stacked $x_{1:K}$ and $z$:
\begin{align}
	\begin{aligned}
		f(z^{\pi}; x_{1:K}^{\pi}, x\com, \theta)^{\pi^{-1}} = f(z; x_{1:K}, x\com, \theta)
		\\
		\forall \text{permutations } \pi
	\end{aligned}
	\label{eq:conditional-nf}
\end{align}
where $z^{\pi}:= (z_{\pi(1)},\ldots,z_{\pi(K)})$ denotes a permuted vector.
We call this an \textbf{invariant conditional normalizing flow model}.
% TODO: better not call it "flow", but flow-based model? density model?
% 
If $K$ is fixed, we call it \textbf{fixed size}, otherwise \textbf{dynamic size}. 
In IMTS forecasting, we have both inputs:
%a variable number of queries $\xq_1,…,\xq_K$ (each a time point and channel),
%for each of which you want an output
%(the predicted value at that time point in that channel) and
%the past observed time series $\xobs$ (see section~\ref{sec:prilims},
%``IMTS probabilistic forecasting problem'').
%So here: 
$(x_1,…x_K):= (\xq_1,…,\xq_K)$, $x^\text{com} := \xobs$.

\paragraph{Invariant conditional normalizing flows via continuous flows.}
Invariant conditional normalizing flow models have been developed
in the literature based on the \textbf{continuous flow} approach
\citep{Chen2018.Neural,Grathwohl2019.Scalable}, 
where the transformation $f$ is specified implicitly by an ordinary
differential equation with time-dependent vector
field $g: \R\times\R^M\rightarrow\R^M$:
\begin{align}
	\begin{aligned}
		f^{-1}(z) := v(1) \quad \text{ with } v : [0,1]\rightarrow\R^K \\
		\text{ being the solution of }
		\frac{\partial v}{\partial\tau} = g(\tau, v(\tau)),
		\quad   v(0)  := z
	\end{aligned}
	\label{eq:cnf}
\end{align}
$\tau$ often is called virtual time to clearly distinguish it from time as
an input variable. 
The vector field $g$ is represented by a parametrized function $g(\tau, v; \theta)$
and then can be learnt. Continuous flow models can be made conditional by
simply adding the predictors $x$ to the inputs of the vector field, too:
$g(\tau, v; x, \theta)$. 
Unconditional structured continuous flow models
can be made permutation invariant by simply making
the vector field permutation equivariant
\citep{Kohler2020.Equivariant,Li2020.Exchangeable,Bilos2021.Normalizing}:
$g(\tau, v^{\pi}; \theta)^{\pi^{-1}} =   g(\tau, v; \theta)$.
To make \textsl{conditional} structured continuous flow models
permutation invariant, the vector field has to be
\textbf{jointly permutation equivariant} in outputs $v$ and predictors $x$:
\begin{align*}
	g(\tau, v^{\pi}; x^{\pi}, \theta)^{\pi^{-1}} & =   g(\tau, v; x, \theta)
\end{align*}
The primary choice for a dynamic size, equivariant, parametrized function
is self attention (\satt):
\begin{align*}
	A(X) &:= XW_\text{Q}(XW_\text{K})^T, \quad
	\\ A^{\text{softmax}}(X) &:= \text{softmax}(A(X))
	\\   \satt(X) & := A^{\text{softmax}}(X)\cdot XW_\text{V}
\end{align*} 
where $X$ is a matrix containing the elements $x_{1:K}$ as rows,
$W_\text{Q},W_\text{K},W_\text{V}$ are parameter matrices (not depending on the number of rows of $X$)
and the softmax is taken rowwise.

Self attention has been used in the literature as is for unconditional
vector fields \citep{Kohler2020.Equivariant,Li2020.Exchangeable,Bilos2021.Normalizing}.
To be used in a conditional vector field, $X$ will have to contain
both, the condition elements $x_{1:K}$ and the base samples $z_{1:K}$ stacked:
\begin{align*}
	X := \left[\begin{array}{cc} x_1^T & z_1
		\\ \vdots & \vdots
		\\ x_K^T & z_K
	\end{array}\right]
\end{align*}




\commentout{
	Now let's find out what the literature means with ``equivariant vector fields'':
	\begin{align*}
		g(\tau, v^{\pi}; x, \theta)^{\pi^{-1}} & =   g(\tau, v; x, \theta)
		\\ \text{or }
		g(\tau, v^{\pi}; x^{\textcolor{red}\pi}, \theta)^{\pi^{-1}} & =   g(\tau, v; x, \theta)
	\end{align*}
	
	
	\cite{Liu2019.Graph}:
	+ dynamic size, equivariant  (graph)
	- unconditional; 
	\cite{Kohler2020.Equivariant}:
	+ equivariant
	= transformation: continuous flow with equivariant vector field
	- unconditional
	\cite{Weilbach2020.Structured}
	- no dynamic size, not equivariant, unconditional
	= transformation: continuous flow with equivari
	ant vector field
	= they use structural zeros in the target covariance matrix ?
	\cite{Li2020.Exchangeable}
	+ dynamic size, permutation equivariant
	= transformation: continuous flow
	+ equivariant transformation: eq. deep set + attention/set transformer
	- not conditional (also see architectures, tab. 3 in the appendix)
	- but they do not have experiments for conditional density estimation, but only
	1. 4.2, fig. 3: conditional point estimation (not elementwise, just a classification)
	2. 4.3, tab. 2 + fig. 4+5: unconditional density estimation
	3. 4.4, fig 6: unconditional density estimation   
	\cite{Bilos2021.Scalablea}
	+ dynamic size, permutation equivariant
	= transformation: continuous flow
	+ equivariant transformation: eq. deep set + attention/set transformer
	+ conditional
	
	
	\cite{Li2020.Exchangeable}
	\cite{Bilos2021.Scalablea}
	
	\cite{Deng2020.Modeling}
}
% \section{Invariant Conditional Normalizing Flow Models via Invertible Self Attention}
\paragraph{Invariant conditional normalizing flows via invertible self attention.}
When using self attention as vector field inside a continuous flow as in the
previous section, then the continuous flow will provide invertibility.
While an elegant and generic approach, continuous flows require
ODE solvers and have been reported to be brittle and not straight-forward
to train. 
% TODO: references
We develop an alternative idea: to make self attention itself invertible
(in the last column of $X$, which contains $z$). Then it can be used
directly, without any need for an ODE wrapper. 
% Unfortunately, self attention is not invertible (in the last column of $X$, which contains $z$).
To get \textbf{invertible self attention (\isatt)} (in the last column), we
i) fix the last row of attention query and key matrices $W_\text{Q}$ and $W_\text{K}$ to zero,
in effect {\em computing the attention matrix $A$ on the conditioners $x_{1:K}$ alone},
ii) fix all but the last rows of $W_\text{V}$ to zero and its last row to
all ones,
in effect {\em using the base sample $z_{1:K}$ alone as attention value},
and
iii) regularize the attention matrix $A$ sufficiently to become invertible (see Section~\ref{sec:Areg_invert_proof}):
\begin{align}
	A^{\text{reg}}(X) & := \frac{1}{\|A(X)\|_2+\epsilon} A(X) + \id      \label{eq:eps}
	\\ \isatt(X) & := A^{\text{reg}}(X_{:,1:|X|{-}1}) X_{:,|X|}
	\label{eq:isatt}
\end{align}
where $\epsilon>0$ is a hyperparameter.
We note that different from a simple linear flow, the slope matrix
$A^{\text{reg}}$ is not a parameter of the model, but computed from the
conditioners $x_{1:K}$.
%
Our approach is different from iTrans attention \citep[fig. 17]{Sukthanker2022.Generative}
that makes attention invertible more easily via
$ A^{\text{iTrans}}:= A^{\softmax}(X) + \id$ using the fact that the spectral radius
$\sigma(A^{\softmax}(X)) \le 1$, but therefore is restricted to non-negative
interaction weights.

% 1. triangular matrix
The attention matrix $A^{\text{reg}}$ will be dense in general and thus slow to
invert, taking $\bigO(K^3)$ operations.
Knothe–Rosenblatt rearrangement~\citep{Villani2009.Optimal}
from optimal transport theory says that 
any two probability distributions on $\R^K$ can be transformed
into each other by flows with a locally triangular Jacobian without
restricting the expressivity of the model.
A triangular slope matrix allows a much more efficient inverse pass, 
as its determinant can be computed in $\bigO(K)$ and linear systems can be solved in $\bigO(K^2)$.
%
% 2. expressivity triangular
%This does not restrict the expressivity of the model, as
%due to the Knothe–Rosenblatt rearrangement~\citep{Villani2009.Optimal}
%from optimal transport theory,

%Note that this does not restrict the expressivity of the model, as the results from optimal transport theory show that any two probability distributions on $\mathbb{R}^K$ can be transformed into each other by flows with locally triangular Jacobian (see Knothe–Rosenblatt rearrangement~\citep{Villani2009.Optimal}).
%
% 3. fixed sorting
Unfortunately, just masking the upper triangular part of the matrix will destroy the
equivariance of the model. We resort to the simplest way to make
a function equivariant: we sort the inputs before passing them into the layer and revert the outputs to the original ordering. We call this approach \textbf{sorted invertible triangular self attention (\stisatt)}:
\begin{align}
	%	\pi &= \operatorname{argsort}(X)   \qquad\text{sort rows based on time and channel}
&	\pi := \argsort (x_1S,\ldots,x_KS) \label{eq:pi}
	\\   
&	A^{\text{tri}}(X)  := \text{softplus-diag}(\text{lower-triang}(A(X))) +\epsilon\id \label{eq:Atri}
	\\ 
&	\stisatt(X)  :=(A^{\text{tri}}(X_{:,1:|X|{-}1}^{\pi}) X_{:,|X|}^{\pi})^{\pi^{-1}} \label{eq:SITA}
	%%	\\ \stisatt(X) & :=P^T(A^{\text{tri}}(P X_{:,1:|X|{-}1}) PX_{:,|X|})
	%	\\ 
	%\operatorname{ITA}(X) & :=(A^{\text{tri}}(X_{:,1:|X|{-}1}) X_{:,|X|})
	%	\\ \stisatt(X) & := P_{\pi^{-1}} \cdot \operatorname{ITA}(P_{\pi} \cdot X)  \qq{where $P_{\pi}$ is the permutation matrix of $\pi$}
\end{align}
%
where $\pi$ operates on the rows of $X$.
%Please note, that different from fixed size functions, where the sorting
%trick easily can be combined with any function, even a fully connected layer,
%for dynamic size functions still precaution is required, here, by using
%an attention mechanism.
Sorting is a simple lexicographic sort along the dimensions of the $x_kS$.
The matrix $S$ allows to specify a sorting criterion, e.g., a permutation
matrix. \hl{As an example, 
For a sequence of numbers in $x$, sort them in ascending order.
If $x$ is a sequence of tuples, prioritize sorting based on
the elements within each tuple (first, second, etc.).
In IMTS with tuple queries, sort first by timestamp,
making triangular matrix correspond to causal attention and 
then by channel.
Note that sorting is unique only when $x$ has unique elements, which holds for our IMTS.}

%\begin{figure}[h]
%	\input{fig/permutation_sort}
%\end{figure}

%This order, or more general $S$, becomes then a hyperparameter of the
% method.

% TODO: Write that we apply in reverse order at the time of training.



==> fig/permutation_sort.tex <==
\begin{tikzpicture}
\node at (0,0) (q) {$\left((1,1), (0,1), (2,0), (3,0), (0,0), (3,1)\right)$};
\node at (0,-1) (pi) {$\left(2, 1,3,4,0,5\right)$};
\node at (0,-2) (sorted_q) {$\left((0,0), (0,1), (1,1), (2,0), (3,0), (3,1)\right)$};
\end{tikzpicture}

==> fig_prop.tex <==



\centering

\resizebox{\linewidth}{0.9\linewidth}    {










\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,971); %set diagram left start at 0, and has height of 971
	
	%Rounded Rect [id:dp9869081262611659] 
	\draw  [fill={rgb, 255:red, 184; green, 224; blue, 242 }  ,fill opacity=1 ] (164.55,213.53) .. controls (164.55,208.33) and (168.76,204.11) .. (173.96,204.11) -- (230.33,204.11) .. controls (235.53,204.11) and (239.74,208.33) .. (239.74,213.53) -- (239.74,241.77) .. controls (239.74,246.97) and (235.53,251.18) .. (230.33,251.18) -- (173.96,251.18) .. controls (168.76,251.18) and (164.55,246.97) .. (164.55,241.77) -- cycle ;
	%Rounded Rect [id:dp7318658333126322] 
	\draw  [fill={rgb, 255:red, 213; green, 232; blue, 20 }  ,fill opacity=0.54 ] (-1.35,86.82) .. controls (-1.35,83.52) and (1.32,80.85) .. (4.63,80.85) -- (108.18,80.85) .. controls (111.48,80.85) and (114.16,83.52) .. (114.16,86.82) -- (114.16,104.75) .. controls (114.16,108.05) and (111.48,110.73) .. (108.18,110.73) -- (4.63,110.73) .. controls (1.32,110.73) and (-1.35,108.05) .. (-1.35,104.75) -- cycle ;
	%Straight Lines [id:da9880705810578669] 
	\draw [line width=1.5]    (54.47,57.69) -- (54.47,76.47) ;
	\draw [shift={(54.47,80.47)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
	%Straight Lines [id:da2710391296046686] 
	\draw [line width=1.5]    (53.69,109.98) -- (53.69,436.45) ;
	%Shape: Ellipse [id:dp3757566350532735] 
	\draw   (190.13,154.06) .. controls (190.13,147.87) and (195.34,142.85) .. (201.76,142.85) .. controls (208.18,142.85) and (213.39,147.87) .. (213.39,154.06) .. controls (213.39,160.25) and (208.18,165.27) .. (201.76,165.27) .. controls (195.34,165.27) and (190.13,160.25) .. (190.13,154.06) -- cycle ;
	%Rounded Rect [id:dp08519407296282444] 
	\draw  [fill={rgb, 255:red, 184; green, 224; blue, 242 }  ,fill opacity=1 ] (164.55,318.12) .. controls (164.55,312.92) and (168.76,308.7) .. (173.96,308.7) -- (230.33,308.7) .. controls (235.53,308.7) and (239.74,312.92) .. (239.74,318.12) -- (239.74,346.36) .. controls (239.74,351.56) and (235.53,355.77) .. (230.33,355.77) -- (173.96,355.77) .. controls (168.76,355.77) and (164.55,351.56) .. (164.55,346.36) -- cycle ;
	%Rounded Rect [id:dp7334652337979062] 
	\draw  [fill={rgb, 255:red, 184; green, 224; blue, 242 }  ,fill opacity=1 ] (164.55,422.71) .. controls (164.55,417.51) and (168.76,413.29) .. (173.96,413.29) -- (230.33,413.29) .. controls (235.53,413.29) and (239.74,417.51) .. (239.74,422.71) -- (239.74,450.95) .. controls (239.74,456.15) and (235.53,460.36) .. (230.33,460.36) -- (173.96,460.36) .. controls (168.76,460.36) and (164.55,456.15) .. (164.55,450.95) -- cycle ;
	%Straight Lines [id:da6045460685509338] 
	\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (199.43,250.43) -- (199.43,305.45) ;
	\draw [shift={(199.43,309.45)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Straight Lines [id:da23274496983403803] 
	\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (199.43,355.02) -- (199.43,410.04) ;
	\draw [shift={(199.43,414.04)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Rounded Rect [id:dp8920901433415311] 
	\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (86.25,140.31) .. controls (86.25,135.12) and (90.46,130.9) .. (95.66,130.9) -- (152.03,130.9) .. controls (157.23,130.9) and (161.45,135.12) .. (161.45,140.31) -- (161.45,168.55) .. controls (161.45,173.75) and (157.23,177.97) .. (152.03,177.97) -- (95.66,177.97) .. controls (90.46,177.97) and (86.25,173.75) .. (86.25,168.55) -- cycle ;
	%Straight Lines [id:da42434088338356424] 
	\draw [line width=1.5]    (52.14,157.05) -- (82.47,157.05) ;
	\draw [shift={(85.47,157.05)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da8833616554220922] 
	\draw [line width=1.5]    (54.47,227.27) -- (162.32,227.27) ;
	\draw [shift={(165.32,227.27)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da9325708570331872] 
	\draw [line width=1.5]    (54.47,331.86) -- (162.32,331.86) ;
	\draw [shift={(165.32,331.86)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da7474070662398151] 
	\draw [line width=1.5]    (54.47,436.45) -- (162.32,436.45) ;
	\draw [shift={(165.32,436.45)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da5221731146111788] 
	\draw [line width=1.5]    (163,156.3) -- (187.13,156.3) ;
	\draw [shift={(190.13,156.3)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da8994306181634497] 
	\draw [line width=1.5]    (200.98,117.45) -- (200.98,141.35) ;
	\draw [shift={(200.98,144.35)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da34838258748735695] 
	\draw [line width=1.5]    (200.98,162.28) -- (200.98,202.61) ;
	\draw [shift={(200.98,205.61)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da10675888685266344] 
	\draw    (241,309) -- (338,55) ;
	%Straight Lines [id:da13532308918002522] 
	\draw    (243,355) -- (336,504) ;
	%Straight Lines [id:da15130763625643806] 
	\draw [line width=1.5]    (200.98,461.11) -- (200.98,501.44) ;
	\draw [shift={(200.98,504.44)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (19.89,-5.99) .. controls (12.65,-2.54) and (6.02,-0.55) .. (0,0) .. controls (6.02,0.55) and (12.65,2.54) .. (19.89,5.99)   ;
	%Straight Lines [id:da2613027323357733] 
	\draw [line width=2.25]    (359,221) -- (399,73) ;
	%Shape: Circle [id:dp3708066969441184] 
	\draw  [line width=2.25]  (399,73) .. controls (399,63.06) and (407.06,55) .. (417,55) .. controls (426.94,55) and (435,63.06) .. (435,73) .. controls (435,82.94) and (426.94,91) .. (417,91) .. controls (407.06,91) and (399,82.94) .. (399,73) -- cycle ;
	%Straight Lines [id:da04157754060471164] 
	\draw [line width=2.25]    (435,73) -- (485.56,102.96) ;
	\draw [shift={(489,105)}, rotate = 210.65] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
	%Straight Lines [id:da877558305574945] 
	\draw [line width=2.25]    (367,240) -- (409,178) ;
	%Shape: Ellipse [id:dp17758723792143272] 
	\draw  [line width=2.25]  (408,147.11) .. controls (415.69,140.81) and (427.03,141.94) .. (433.33,149.63) .. controls (439.63,157.32) and (438.5,168.66) .. (430.81,174.96) .. controls (423.12,181.26) and (411.78,180.13) .. (405.48,172.44) .. controls (399.18,164.75) and (400.31,153.4) .. (408,147.11) -- cycle ;
	%Straight Lines [id:da6739006162867851] 
	\draw [line width=2.25]    (436.81,162.96) -- (488.59,131.1) ;
	\draw [shift={(492,129)}, rotate = 148.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
	%Shape: Circle [id:dp9055928464958285] 
	\draw  [line width=2.25]  (533,117) .. controls (533,104.3) and (522.7,94) .. (510,94) .. controls (497.3,94) and (487,104.3) .. (487,117) .. controls (487,129.7) and (497.3,140) .. (510,140) .. controls (522.7,140) and (533,129.7) .. (533,117) -- cycle ;
	%Shape: Circle [id:dp6865950449243752] 
	\draw  [line width=2.25]  (587,116) .. controls (587,107.99) and (593.49,101.5) .. (601.5,101.5) .. controls (609.51,101.5) and (616,107.99) .. (616,116) .. controls (616,124.01) and (609.51,130.5) .. (601.5,130.5) .. controls (593.49,130.5) and (587,124.01) .. (587,116) -- cycle ;
	%Straight Lines [id:da2999066652280171] 
	\draw [line width=2.25]    (533,117) -- (583,116.07) ;
	\draw [shift={(587,116)}, rotate = 178.94] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
	%Shape: Circle [id:dp3961668222159478] 
	\draw  [line width=2.25]  (581.5,280) .. controls (581.5,268.95) and (590.45,260) .. (601.5,260) .. controls (612.55,260) and (621.5,268.95) .. (621.5,280) .. controls (621.5,291.05) and (612.55,300) .. (601.5,300) .. controls (590.45,300) and (581.5,291.05) .. (581.5,280) -- cycle ;
	%Straight Lines [id:da4499556764453696] 
	\draw [line width=2.25]    (367,250) -- (477.14,276.82) ;
	\draw [shift={(482,278)}, rotate = 193.68] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
	%Shape: Circle [id:dp4736721163591049] 
	\draw  [line width=2.25]  (482,278) .. controls (482,263.64) and (493.64,252) .. (508,252) .. controls (522.36,252) and (534,263.64) .. (534,278) .. controls (534,292.36) and (522.36,304) .. (508,304) .. controls (493.64,304) and (482,292.36) .. (482,278) -- cycle ;
	%Straight Lines [id:da026020652082648255] 
	\draw [line width=2.25]    (369,261) -- (478.12,349.84) ;
	\draw [shift={(482,353)}, rotate = 219.15] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
	%Shape: Ellipse [id:dp34265448540795385] 
	\draw  [line width=2.25]  (487,338.11) .. controls (494.69,331.81) and (506.03,332.94) .. (512.33,340.63) .. controls (518.63,348.32) and (517.5,359.66) .. (509.81,365.96) .. controls (502.12,372.26) and (490.78,371.13) .. (484.48,363.44) .. controls (478.18,355.75) and (479.31,344.4) .. (487,338.11) -- cycle ;
	%Shape: Circle [id:dp3096184235815087] 
	\draw  [line width=2.25]  (581,358) .. controls (581,346.95) and (589.95,338) .. (601,338) .. controls (612.05,338) and (621,346.95) .. (621,358) .. controls (621,369.05) and (612.05,378) .. (601,378) .. controls (589.95,378) and (581,369.05) .. (581,358) -- cycle ;
	%Shape: Circle [id:dp5257028517310518] 
	\draw  [line width=2.25]  (585,437) .. controls (585,425.95) and (593.95,417) .. (605,417) .. controls (616.05,417) and (625,425.95) .. (625,437) .. controls (625,448.05) and (616.05,457) .. (605,457) .. controls (593.95,457) and (585,448.05) .. (585,437) -- cycle ;
	%Straight Lines [id:da5854210838879303] 
	\draw [line width=2.25]    (601.5,46.93) -- (601.5,97.5) ;
	\draw [shift={(601.5,101.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Straight Lines [id:da6152155476429053] 
	\draw [line width=2.25]    (601.5,130.5) -- (601.5,256) ;
	\draw [shift={(601.5,260)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Straight Lines [id:da24244533197769513] 
	\draw [line width=2.25]    (534,278) -- (577.5,279.83) ;
	\draw [shift={(581.5,280)}, rotate = 182.41] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
	%Straight Lines [id:da8129378002559668] 
	\draw [line width=2.25]    (519,351) -- (577.03,357.55) ;
	\draw [shift={(581,358)}, rotate = 186.44] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
	%Straight Lines [id:da7996500157921844] 
	\draw [line width=2.25]    (601.5,300) -- (601.5,334) ;
	\draw [shift={(601.5,338)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Straight Lines [id:da31599900819709315] 
	\draw [line width=2.25]    (601,378) -- (601,412) ;
	\draw [shift={(601,416)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Straight Lines [id:da595907625333651] 
	\draw [line width=2.25]    (605,457) -- (605,507.57) ;
	\draw [shift={(605,511.57)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (24.48,-7.37) .. controls (15.57,-3.13) and (7.41,-0.67) .. (0,0) .. controls (7.41,0.67) and (15.57,3.13) .. (24.48,7.37)   ;
	%Rounded Rect [id:dp3894807850652031] 
	\draw   (326,98.2) .. controls (326,62.74) and (354.74,34) .. (390.2,34) -- (582.8,34) .. controls (618.26,34) and (647,62.74) .. (647,98.2) -- (647,462.8) .. controls (647,498.26) and (618.26,527) .. (582.8,527) -- (390.2,527) .. controls (354.74,527) and (326,498.26) .. (326,462.8) -- cycle ;
	
	% Text Node
	\draw (17.01,31.62) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$(x\obs,x\qu)$};
	% Text Node
	\draw (43.18,84.66) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$\qem$};
	% Text Node
	\draw (193.08,83.91) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$\mathbf{y}$};
	% Text Node
	\draw (192.97,142.93) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {${-}$};
	% Text Node
	\draw (180.96,214.14) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$f^{( 1)}$};
	% Text Node
	\draw (181.52,318.73) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$f^{( l)}$};
	% Text Node
	\draw (181.75,424.34) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$f^{( L)}$};
	% Text Node
	\draw (104.24,140.43) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$f_{\mu }$};
	% Text Node
	\draw (21.52,130.06) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$x$};
	% Text Node
	\draw (204.44,167.83) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$y^{( 1)}$};
	% Text Node
	\draw (205,272.42) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$y^{( l)}$};
	% Text Node
	\draw (204.22,377.01) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$y^{( L)}$};
	% Text Node
	\draw (138.59,499.53) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$y^{( L+1)} \ =\ \mathbf{z}$};
	% Text Node
	\draw (323.28,226.44) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$\mathbf{H}$};
	% Text Node
	\draw (404,62) node [anchor=north west][inner sep=0.75pt]   [font=\huge] {$Q$};
	% Text Node
	\draw (413,152.11) node [anchor=north west][inner sep=0.75pt]   [font=\huge] {$K$};
	% Text Node
	\draw (491,110.11) node [anchor=north west][inner sep=0.75pt]   [font=\huge] {$A(Q,K)$};
	% Text Node
	\draw (595,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {X};
	% Text Node
	\draw (499,271) node [anchor=north west][inner sep=0.75pt]   [align=left] {expsc};
	% Text Node
	\draw (483,343) node [anchor=north west][inner sep=0.75pt]   [align=left] {tras};
	% Text Node
	\draw (588,271) node [anchor=north west][inner sep=0.75pt]   [align=left] {cdot};
	% Text Node
	\draw (595,349) node [anchor=north west][inner sep=0.75pt]   [align=left] {+};
	% Text Node
	\draw (593,428) node [anchor=north west][inner sep=0.75pt]   [align=left] {act};
	% Text Node
	\draw (553.54,463.42) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$y^{( l)}$};
	% Text Node
	\draw (550.54,44.42) node [anchor=north west][inner sep=0.75pt]  [font=\huge]  {$y^{( l)}$};
	
	
\end{tikzpicture}


}

==> impactstatement.tex <==
\section*{Impact statements}
This paper presents work whose goal is to advance the field of Machine Learning.
There are many potential societal consequences of our work,
none which we feel must be specifically highlighted here.

==> invertible-self-attention.tex <==

% \section{Invariant Conditional Normalizing Flow Models via Continuous Flows}
\section{Invariant Conditional Normalizing Flow Models}
% \subsection{Delineation from Related Work}
\paragraph{Normalizing flows.}
While parametrizing a specific distribution such as the Normal
% TODO: reference
is a simple and robust approach to probabilistic forecasting
that can be added on top of any point forecasting model
(for marginal distributions or fixed-size queries at least),
such models are less suited for targets having a more
complex distribution. Then typically normalizing flows are
used \cite{Rippel2013.Highdimensional, Papamakarios2021.Normalizing}.
A normalizing flow is an (unconditional) density model for 
variables $y\in\R^K$ consisting of
  a simple base distribution,
    typically a standard normal $p_Z(z):= \normal(z; 0_K, \id_{K\times K})$, and
  an invertible, differentiable, parametrized map
  $f(z; \theta)$; then
\begin{align}
    \hat p(y; \theta) :=
       p_Z(f^{-1}(y; \theta)) \left| \text{det}\left(\frac{\partial f^{-1}(y; \theta)}{\partial y}\right) \right|
       \label{eq:nf}
\end{align}
is a proper density, i.e., integrates to 1, and can be fitted to data minimizing
negative log likelihood via gradient descent algorithms.
A normalizing flow can be conditioned on predictor variables $x\in\R^M$
by simply making $f$ dependent on predictors $x$, too: $f(z; x, \theta)$. 
$f$ then has to be invertible w.r.t. $z$ for any $x$ and $\theta$ \citep{BR18}.

\paragraph{Invariant conditional normalizing flows.}
A conditional normalizing flow represents an invariant
conditional distribution in the sense of eq.~\ref{eq:invariant},
if
  i) its predictors $x$ also can be grouped into $K$ elements $x_1,\ldots,x_K$
     and possibly common elements $x\com$:
        $x =(x_1,\ldots,x_K,x\com)$, and
  ii) its transformation $f$ is equivariant in stacked $x_{1:K}$ and $z$:
\begin{align}
  f(z^{\pi}; x_{1:K}^{\pi}, x\com, \theta)^{\pi^{-1}} = f(z; x_{1:K}, x\com, \theta)
   \quad\forall \text{permutations } \pi
\end{align}
 where $z^{\pi}:= (z_{\pi(1)},\ldots,z_{\pi(K)})$ denotes a permuted vector.
We call this an \textbf{invariant conditional normalizing flow model}.
% TODO: better not call it "flow", but flow-based model? density model?
% 
If $K$ is fixed, we call it \textbf{fixed size}, otherwise \textbf{dynamic size}.

\paragraph{Invariant conditional normalizing flows via continuous flows.}
Invariant conditional normalizing flow models have been developed
in the literature based on the \textbf{continuous flow} approach
\citep{Chen2018.Neural, Grathwohl2019.Scalable}, 
where the transformation $f$ is specified implicitly by an ordinary
differential equation with time-dependent vector
field $g: \R\times\R^M\rightarrow\R^M$:
\begin{align*}
    f^{-1}(z) & := v(1)
\quad \text{with } v : [0,1]\rightarrow\R^K
  \text{ being the solution of }
  \frac{\partial v}{\partial\tau} = g(\tau, v(\tau)),
       \quad   v(0)  := z
\end{align*}
$\tau$ often is called virtual time to clearly distinguish it from time as
an input variable. 
The vector field $g$ is represented by a parametrized function $g(\tau, v; \theta)$
and then can be learnt. Continuous flow models can be made conditional by
simply adding the predictors $x$ to the inputs of the vector field, too:
  $g(\tau, v; x, \theta)$. 
Unconditional structured continuous flow models
can be made permutation invariant by simply making
the vector field permutation equivariant
\citep{Kohler2020.Equivariant,Li2020.Exchangeable,Bilos2021.Scalablea}:
$g(\tau, v^{\pi}; \theta)^{\pi^{-1}} =   g(\tau, v; \theta)$.
To make \textsl{conditional} structured continuous flow models
permutation invariant, the vector field has to be
\textbf{jointy permutation equivariant} in outputs $v$ and predictors $x$:
\begin{align*}
  g(\tau, v^{\pi}; x^{\pi}, \theta)^{\pi^{-1}} & =   g(\tau, v; x, \theta)
\end{align*}

The primary choice for a dynamic size, equivariant, parametrized function
is self attention:
\begin{align*}
    A(X) &:= XQ(XK)^T, \quad
           A^{\text{softmax}}(X) := \text{softmax}(A(X))
 \\   \text{satt}(X; Q,K,V) & := A^{\text{softmax}}(X) \, XV
\end{align*}
where $X$ is a matrix containing the elements $x_{1:K}$ as rows,
$Q,K,V$ are parameter matrices (not depending on the number of rows of $X$)
and the softmax is taken rowwise.

Self attention has been used in the literature as is for unconditional
vector fields \citep{Kohler2020.Equivariant,Li2020.Exchangeable,Bilos2021.Scalablea}.
To be used in a conditional vector field, $X$ will have to contain
both, the condition elements $x_{1:K}$ and the base samples $z_{1:K}$ stacked:
\begin{align*}
   X := \left[\begin{array}{cc} x_1^T & z_1
                                        \\ \vdots & \vdots
                                        \\ x_K^T & z_K
                   \end{array}\right]
\end{align*}


  

\commentout{
Now let's find out what the literature means with ``equivariant vector fields'':
\begin{align*}
     g(\tau, v^{\pi}; x, \theta)^{\pi^{-1}} & =   g(\tau, v; x, \theta)
\\ \text{or }
     g(\tau, v^{\pi}; x^{\textcolor{red}\pi}, \theta)^{\pi^{-1}} & =   g(\tau, v; x, \theta)
\end{align*}


  \cite{Liu2019.Graph}:
+ dynamic size, equivariant  (graph)
- unconditional; 
\cite{Kohler2020.Equivariant}:
+ equivariant
= transformation: continuous flow with equivariant vector field
- unconditional
\cite{Weilbach2020.Structured}
- no dynamic size, not equivariant, unconditional
= transformation: continuous flow with equivari
ant vector field
= they use structural zeros in the target covariance matrix ?
\cite{Li2020.Exchangeable}
+ dynamic size, permutation equivariant
= transformation: continuous flow
+ equivariant transformation: eq. deep set + attention/set transformer
- not conditional (also see architectures, tab. 3 in the appendix)
- but they do not have experiments for conditional density estimation, but only
  1. 4.2, fig. 3: conditional point estimation (not elementwise, just a classification)
  2. 4.3, tab. 2 + fig. 4+5: unconditional density estimation
  3. 4.4, fig 6: unconditional density estimation   
\cite{Bilos2021.Scalablea}
+ dynamic size, permutation equivariant
= transformation: continuous flow
+ equivariant transformation: eq. deep set + attention/set transformer
+ conditional


\cite{Li2020.Exchangeable}
\cite{Bilos2021.Scalablea}

\cite{Deng2020.Modeling}
}

% \section{Invariant Conditional Normalizing Flow Models via Invertible Self Attention}
\paragraph{Invariant conditional normalizing flows via invertible self attention.}
When using self attention as vector field inside a continuous flow as in the
previous section, then the continuous flow will provide invertibility.
While an elegant and generic approach, continuous flows require
ODE solvers and have been reported to be brittle and not straight-forward
to train. 
% TODO: references
We develop an alternative idea: to make self attention itself invertible
(in the last column of $X$, which contains $z$). Then it can be used
directly, without any need for an ODE wrapper. 
% Unfortunately, self attention is not invertible (in the last column of $X$, which contains $z$).
To get \textbf{invertible self attention} (in the last column), we
i) fix the last row of attention queries $Q$ and keys $K$ to zero,
  in effect computing the attention matrix $A$ on the conditioners $x_{1:K}$ alone,
ii) fix all but the last rows of attention values $V$ to zero and its last row to
  all ones,
  in effect using the base sample $z_{1:K}$ alone as attention value,
  and
iii) regularize the attention matrix $A$ sufficiently to become invertible:
\begin{align}
       A^{\text{reg}}(X) & := \frac{1}{\sigma(A(X))+\epsilon} A(X) + \id      
  \\ \text{isatt}(X; Q,K) & := A^{\text{reg}}(X_{1:|X|{-}1,.}) X_{|X|,.}
  \label{eq:isatt}                            
\end{align}
where $\sigma$ denotes the spectral radius and $\epsilon>0$ a small constant.
Please note, that different from a simple linear flow, the slope matrix
$A^{\text{reg}}$ is not a parameter of the model, but computed from the
conditioners $x_{1:K}$.
%
Our approach is different from iTrans attention \citep[fig. 17]{Sukthanker2022.Generative}
that makes attention invertible more easily via
$ A^{\text{iTrans}}:= A^{\softmax}(X) + \id$ using the fact that
$\sigma(A^{\softmax}(X)) < 1$, but therefore is restricted to non-negative
interaction weights.

% 2. fixed sorting
The attention matrix $A^{\text{reg}}$ will be dense in general and thus slow to
invert. Following ideas for autoregressive flows and coupling layers,
% TODO: references
a triangular slope matrix would be way faster to invert. Unfortunately,
just masking the upper triangular part of the matrix will destroy the
equivariance of the approach. We resort to the most simple way to make
a function equivariant: we fix the order of its input elements to
get \textbf{sorted triangular invertible self attention}:
\begin{align*}
    \pi & := \argsort (x_1S,\ldots,x_KS)
\\ &  A^{\text{tri}}(X) := \text{softplus-diag}(\text{lower-triangular}(A(X)) +\epsilon\id
  \\ \text{stisatt}(X; Q,K,S) & :=(A^{\text{tri}}(X_{1:|X|{-}1,.}^{\pi}) X_{|X|,.}^{\pi})^{\pi^{-1}}
\end{align*}
where $\pi$ operates on the rows of $X$. 
Please note, that different from fixed size functions, where the sorting
trick easily can be combined with any function, even a fully connected layer,
for dynamic size functions still precaution is required, here, by using
an attention mechanism.
Sorting is a simple lexicographic sort along the dimensions of the $x_kS$.
The matrix $S$ allows to specify a sorting criterion, e.g., a permutation
matrix. For example, we will sort time series queries first by time stamp,
so that the triangular matrix corresponds to a causal attention,
second by channel, fixing some order of the channels.
This order, or more general $S$, becomes then a hyperparameter of the
method.
% todo: discuss BN; graphical flow paper.

% 3. learned sorting
To avoid this hyperparamerter and even allow different sorting criteria
for different instances, one can parametrize $S$ as a function
of $X_{1:|X|{-}1,.}$ (\textbf{learned sorted triangular invertible self attention}).



\commentout{
Sorting introduces a hyperparameter: the sorting criterion, here
represented by matrix $S$. A simple
lexicographic sort along the dimensions of the $x_k$ is most
simple; but even then the order of the dimensions of the $x_k$
become a hyperparameter.
% todo: discuss BN; graphical flow paper.

\bigskip\bigskip

% 3. fixed sorting (of the queries / condition elements; or of the latent elements?)
\begin{align*}
    \pi & := \argsort (x_{1:K})
  \\ f(z; x, x\com, \theta) :=
          \tilde f(z^{\pi}; x^{\pi}, x\com, \theta)^{\pi^{-1}}
\end{align*}
with $\tilde f$ any function.
}


\commentout{
conditional and (permutation) equivariant
  !=
conditional  equivariant   (better name?)


autoreg, coupling
residual
linear
cont

equivariant:
- sum of elementwise and invariant (deepset)
- attention
\begin{align*}
  A := 
\end{align*}


- graph segmentation
- vertex-wise graph regression / vertex regression
- probabilistic 



\cite{Bose2021.Equivariant}  % 3 general approaches



\cite{Wehenkel2021.Graphical, Wehenkel2020.You}

\cite{GarciaSatorras2021.Equivariant, Satorras2021.Equivariant}
% euclidean
\cite{Kohler2020.Equivariant} % euclidean?
- equivariant flow = equivariant transformation


\cite{Bilos2021.Scalablea}  % invariant

\cite{Liu2019.Graph}   % ??
}

% \marginpar{make 5.3 the next top-level section, and then add a section 6 on stitching everything together}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "profiti-lst"
%%% End:


==> prilims.tex <==
\section{Problem Setting \&\ Analysis}
\label{sec:prilims}

%\begin{figure}[h]
%	\scriptsize
%	\centering
%	\input{fig/prilim_fig}
%\end{figure}

\paragraph{The IMTS Forecasting Problem.}
\label{sec:imts_forec}

An \textbf{irregularly sampled multivariate times series with missing values}
(called briefly just \textbf{IMTS} in the following),
is a finite sequence 
$x\obs = \left((t_i\obs, c_i\obs, o_i\obs)\right)_{i=1:I}$
of unique triples, 
where
$t_i\obs \in \R$ denotes the time,
$c_i\obs \in \{1,...,C\}$ the channel and
$o_i\obs \in \R$ the value of an observation,  % TODO: consider v_n ?
$I\in\N$ the total number of observations across all channels
and $C\in\N$ the number of channels.
Let $\text{TS}(C):=(\R\times\{1,\ldots,C\}\times\R)^*$ denote the
space of all IMTS with $C$ channels. 
We use $(\cdot)^*$ to indicate the space of finite sequences of arbitrary length.

An \textbf{IMTS query} is a finite sequence
$x\qu = \left((t_k\qu, c_k\qu)\right)_{k=1:K} \in \text{Q}(C):= (\R\times\{1,\ldots,C\})^*$
of just time points and channels (also unique), a sequence $y\in\R^K$ we call
an answer and denote by
$\text{QA}(C):= \{ (x\qu, y)\in \text{Q}(C)\times\R^* \mid  |x\qu| =  |y| \}$
the space of all queries and possible answers.

The \textbf{IMTS probabilistic forecasting problem} then
is, given a dataset
$\D^\text{train}:= \left((x\obs_n, x\qu_n, y_n)\right)_{n=1:N}\in \text{TS}(C)\times\text{QA}(C)$
of triples of time series, queries and answers from an unknown distribution $p$
(with earliest query timepoint is beyond the latest observed timepoint for series $n$, $\min_k t\qu_{n,k} > \max_i t\obs_{n,i}$),
to find a model $\hat p$ that maps each observation/query pair $(x\obs,x\qu)$
to a joint density over answers,
$\hat p(y_1, \ldots, y_K \mid x\obs, x\qu)$, such that the expected joint negative
log likelihood is minimal:
\begin{align*}
	\ell^\text{jNLL}(\hat p; p) := - {\mathbb E}_{(x\obs,x\qu,y)\sim p} \log \hat p(y \mid x\obs, x\qu)
\end{align*}
Please note, that the number $C$ of channels is fixed, but
the number $I$ of past observations and
the number $K$ of future observations queried
may vary over instances $(x\obs,x\qu,y)$.
% 
If query sizes $K$ vary, instead of (joint) negative log likelihood one also can normalize
by query size to make numbers comparable over different series and limit
the influence of large queries, the \textbf{normalized joint negative
	log likelihood} njNLL:
\begin{align}
	\ell^\text{njNLL}(\hat p; p)
	& :=- \mathop{\mathbb{E}}_{(x\obs, x\qu, y)\sim p} \frac{1}{|y|} \log \hat p(y \mid x\obs, x\qu)
	\label{eq:njnl}
\end{align}

\paragraph{Problem Analysis and Characteristics.}
% maybe "property" instead of  "requirement" ? 
As the problem is not just an (unconditioned) density estimation problem,
but the distribution of the outputs depends on both, the past observations
and the queries, a \textbf{conditional density model} is required 
(\textbf{requirement 1}).
% puh, sounds super lame.

% delineation from marginal probabilistic forecasting.
A crucial difference from many settings addressed in the related work
% TODO: add references
is that we look for probabilistic models of the \textbf{joint distribution} of all
queried observation values $y_1, \ldots, y_K$, not just at
the \textbf{single variable marginal distributions}
$p(y_k \mid x\obs, x\qu_k)$ (for $k=1{:}K$).
The problem of marginal distributions is a special case of our formulation
where all queries happen to have just one element (always $K=1$).

So for joint probabilistic forecasting of IMTS,
models need to output densities on a \textbf{variable number of
	variables} (\textbf{requirement 2}).

Furthermore, whenever two query elements get swapped,
a generative model should swap its output accordingly,
a density model should yield the same density value, 
i.e.,
the model should be \textbf{permutation invariant} (\textbf{requirement 3}):
for every permutation $\pi$:
\begin{align}
	&\hat p(y_1,\ldots,y_K \mid x\obs,x\qu_1,\ldots,x\qu_K)
	 = \notag \\
	&\hat p(y_{\pi(1)},\ldots,y_{\pi(K)} \mid x\obs,x\qu_{\pi(1)},\ldots,x\qu_{\pi(K)})
	\label{eq:invariant}
\end{align}

Permutation invariant models are studied for IMTS classification~\citep{Horn2020.Set,Yalavarthi2022.DCSF}
and equivariant models for interpolation~\citep{Yalavarthi2023.Tripletformer} 
and forecasting~\citep{Yalavarthi2024.GraFITi}; and achieve state-of-the-art results.
To the best of our knowledge, we are the first to explore permutation equivariant 
generative model forecasting.
Note that permutation equivariance is crucial w.r.t. channels
but is not a necessary for time points due to the causal nature of the series.
But it is a very successful property of most state-of-the-art models in vision and time series~\citep{Zhou2021.Informer,Dosovitskiy2020.Image}. 
All queries carry the time point as an attribute (in $q_k$),
like positional encodings in transformers, so that the model can
detect and represent temporal dependencies, of course.



% also: consistent w.r.t. duplicate query elements?

==> shiesh_figure.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			xlabel=$x$,
			ylabel=$\alpha(u,t)$,
			legend pos=north west,
			title={Plot of $\alpha(u,t) = \arcsinh(\exp(t)\sinh(x))$},
			ymin=-10, ymax=10,
			grid=both,
			width=0.45\textwidth,
			]
			
			\foreach \t in {0,1}{
				\addplot[color=blue, domain=-5:5, samples=100] {sinh(exp(\t)*sinh(x))};
				\addlegendentry{$t=0$};
			}
			
		\end{axis}
	\end{tikzpicture}
	%
%	\begin{tikzpicture}
%		\begin{axis}[
%			xlabel=$u$,
%			ylabel=$\frac{\partial}{u}(\alpha(u,t))$,
%			legend pos=south east,
%			title={$\frac{\partial}{u}(\alpha(u,t)) = \frac{\exp(t)\cosh(u)}{\sqrt{1 + (\exp(t)\sinh(u))^2}}$},
%			ymin=0, ymax=5,
%			grid=both,
%			width=0.45\textwidth,
%			]
%			
%			\foreach \t in {0,1,2,5,10}{
%				\addplot[color=red, domain=-5:5, samples=100] {exp(\t)*cosh(x)/(sqrt(1 + (exp(\t)*sinh(x))^2))};
%				\addlegendentry{$t=\t$};
%			}
%			
%		\end{axis}
%	\end{tikzpicture}
\end{figure}

